A Policy Profile for Croissant: Refusal as a Property of the Dataset

Croissant is the de facto machine-readable descriptor for ML datasets: JSON-LD over schema.org. Since version 1.1 it also carries data use conditions, recommending DUO and ODRL for them. What no version specifies is how any of them is evaluated: no decision procedure, no bound on evaluation cost, no outcome for a condition an implementation cannot evaluate, no record of what was checked, and nothing on composition with caller-side authority. We supply that half. An additive profile lets a dataset declare the operations it admits and the conditions under which it admits them, over a closed set of five operators whose decision procedure is given in full, so a gate decides from the descriptor alone and records what it checked. Two corpora evaluate it and their evidence is kept apart. Three descriptors that gated a real nf-core pipeline give the deployment result: decisions from a profile document match the gate's native descriptor record for record, stripping the layer leaves a valid Croissant document, and the added cost is 11.7 $\mu$s against a 119 $\mu$s decision. A corpus generated from the profile's grammar gives the breadth, covering every operator, refusal class and conformance clause. Across its valid cases, 552 complete decision records agree three ways -- native descriptor, profile terms, and the same policy as ODRL in usageInfo. The carrier is therefore not the contribution; the evaluation semantics is. Finally, caller-bound and data-bound policies range over non-overlapping state spaces, so neither permit set contains the other.

==> shared-preamble.tex <==

\usepackage{tikz}
\usetikzlibrary{arrows.meta,positioning,fit,backgrounds}

\makeatletter
\DeclareRobustCommand{\code}[1]{\texttt{\frenchspacing\let\dk@prev\relax\dk@codebrk#1\@nil}}
\def\dk@codebrk{\futurelet\dk@peek\dk@codebrk@i}
\def\dk@codebrk@i{%
  \ifx\dk@peek\@sptoken
    \expandafter\dk@codebrk@sp
  \else
    \expandafter\dk@codebrk@tok
  \fi}
\expandafter\def\expandafter\dk@codebrk@sp\space{ \let\dk@prev\relax\dk@codebrk}
\def\dk@codebrk@tok#1{%
  \ifx#1\@nil\else
    \ifx\dk@prev\relax\else\dk@codepen{#1}\fi
    #1\let\dk@prev#1%
    \expandafter\dk@codebrk
  \fi}
\def\dk@codepen#1{%
  \ifx\dk@prev.\penalty50 \else
  \ifx\dk@prev:\penalty50 \else
  \ifx\dk@prev/\penalty50 \else
  \ifx\dk@prev-\penalty50 \else
  \dk@ifupper{#1}{\penalty100 }{\penalty900 }\fi\fi\fi\fi}
\def\dk@ifupper#1#2#3{%
  \ifcat a\noexpand#1%
    \ifnum\lccode`#1=`#1 #3\else #2\fi
  \else #3\fi}
\makeatother

\emergencystretch=1.5em
\newcommand{\us}{\,\mbox{\textmu s}}

